Local statistical moments to capture Kramers-Moyal coefficients

This study introduces an innovative local statistical moment approach for estimating Kramers-Moyal coefficients, effectively bridging the gap between nonparametric and parametric methodologies. These coefficients play a crucial role in characterizing stochastic processes. Our proposed approach provides a versatile framework for localized coefficient estimation, combining the flexibility of nonparametric methods with the interpretability of global parametric approaches. We showcase the efficacy of our approach through use cases involving both stationary and non-stationary time series analysis. Additionally, we demonstrate its applicability to real-world complex systems, specifically in the energy conversion process analysis of a wind turbine.

==> bib.tex <==
@article{nikakhtar2023data,
	title={Data-driven reconstruction of stochastic dynamical equations based on statistical moments},
	author={Nikakhtar, Farnik and Parkavousi, Laya and Sahimi, Muhammad and Tabar, M Reza Rahimi and Feudel, Ulrike and Lehnertz, Klaus},
	journal={New Journal of Physics},
	volume={25},
	number={8},
	pages={083025},
	year={2023},
	publisher={IOP Publishing}
}
